Inferring Needless Write Memory Accesses on Ethereum Bytecode (Extended Version)

Efficiency is a fundamental property of any type of program, but it is even more so in the context of the programs executing on the blockchain (known as smart contracts). This is because optimizing smart contracts has direct consequences on reducing the costs of deploying and executing the contracts, as there are fees to pay related to their bytes-size and to their resource consumption (called gas). Optimizing memory usage is considered a challenging problem that, among other things, requires a precise inference of the memory locations being accessed. This is also the case for the Ethereum Virtual Machine (EVM) bytecode generated by the most-widely used compiler, \texttt{solc}, whose rather unconventional and low-level memory usage challenges automated reasoning. This paper presents a static analysis, developed at the level of the EVM bytecode generated by \texttt{solc}, that infers write memory accesses that are needless and thus can be safely removed. The application of our implementation on more than 19,000 real smart contracts has detected about 6,200 needless write accesses in less than 4 hours. Interestingly, many of these writes were involved in memory usage patterns generated by \texttt{solc} that can be greatly optimized by removing entire blocks of bytecodes. To the best of our knowledge, existing optimization tools cannot infer such needless write accesses, and hence cannot detect these inefficiencies that affect both the deployment and the execution costs of Ethereum smart contracts.

==> defs.tex <==
% Macros

\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}
\definecolor{halfgray}{gray}{0.55}
\definecolor{ipythonframe}{RGB}{207, 207, 207}

\definecolor{ckeyword}{HTML}{7F0055}
\definecolor{ccomment}{HTML}{3F7F5F}
\definecolor{cnumber}{HTML}{2A0099}
\definecolor{pblue}{rgb}{0.13,0.13,1}
\definecolor{pgreen}{rgb}{0,0.5,0}
\definecolor{pred}{rgb}{0.9,0,0}
\definecolor{pgrey}{rgb}{0.46,0.45,0.48}

\definecolor[named]{ACMBlue}{cmyk}{1,0.1,0,0.1}
\definecolor[named]{ACMYellow}{cmyk}{0,0.16,1,0}
\definecolor[named]{ACMOrange}{cmyk}{0,0.42,1,0.01}
\definecolor[named]{ACMRed}{cmyk}{0,0.90,0.86,0}
\definecolor[named]{ACMLightBlue}{cmyk}{0.49,0.01,0,0}
\definecolor[named]{ACMGreen}{cmyk}{0.20,0,1,0.19}
\definecolor[named]{ACMPurple}{cmyk}{0.55,1,0,0.15}
\definecolor[named]{ACMDarkBlue}{cmyk}{1,0.58,0,0.21}

\def\lstlistingautorefname{Code}
\renewcommand{\lstlistingname}{Code}

\lstdefinelanguage{Solidity} {
  keywords={typeof, modifier, function, public, returns, external,
  contract, new, true, false, private, catch, function, null, throw, catch, switch, var, if, in, while, do, else, case, break},
  ndkeywords={bool, mapping, bytes32, string},
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{ccomment}\ttfamily,
  string=[b]",
  showstringspaces=false,
  morestring=[b]',
  showspaces=false,
  showtabs=false,  breaklines=true,
  morekeywords={function, contract, returns},
  breakatwhitespace=true,
  lineskip=-0.6pt,
  basewidth={0.54em, 0.4em},
  basicstyle=\scriptsize\ttfamily,
  keywordstyle={\color{ckeyword}\scriptsize\bfseries},
  ndkeywordstyle={\color{black}\scriptsize\bfseries},
  commentstyle={\color{ccomment}\itshape},
  stringstyle={\color{pgreen}},
  numberstyle={\scriptsize\color{cnumber}\ttfamily},
  moredelim=[il][\textcolor{pgrey}]{$$},
  moredelim=[is][\textcolor{pgrey}]{\%\%}{\%\%},
}

\newtheorem{example}{Example}

\newcommand{\scode}[1]{\lstinline[language=Solidity,basicstyle=\small\ttfamily]{#1}}
\newcommand{\code}[1]{\scode{#1}}
\newcommand{\mcode}[1]{\text{\small{\scode{#1}}}}
\newcommand{\evmcode}[1]{\text{\scriptsize{\scode{#1}}}}

\newcommand{\lstcode}[1]{\small\texttt{#1}}

%\renewcommand{\arraystretch}{1.5}

%\usetikzlibrary{shadows}
%\usetikzlibrary{calc}

\newcommand*{\github}{\textsf{github}\xspace}

\definecolor{shadecolor}{gray}{1.00}
\definecolor{ddarkgray}{gray}{0.75}
\definecolor{darkgray}{gray}{0.30}
\definecolor{light-gray}{gray}{0.87}
\newcommand{\whitebox}[1]{\colorbox{white}{#1}}
\newcommand{\graybox}[1]{\colorbox{light-gray}{#1}}
\newcommand{\darkgraybox}[1]{\colorbox{ddarkgray}{#1}}
\newcommand{\gbm}[1]{\graybox{${#1}$}}

\newcommand{\fstar}{\text{F}^{\star}}
\newcommand{\etc}{\emph{etc}}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\Ie}{\emph{I.e.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\Eg}{\emph{E.g.}\xspace}
\newcommand{\vs}{\emph{vs.}\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}
\newcommand{\adhoc}{\emph{ad hoc}\xspace}
\newcommand{\viz}{\emph{viz.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\wrt}{\emph{wrt.}\xspace}
\newcommand{\Iff}{\emph{iff}\xspace}
\newcommand{\loef}{L\"{o}f}

\newcommand{\mute}[1]{{#1}}
\newcommand{\ea}[1]{\mute{\textcolor{ACMGreen}{(Elvira: {#1})}}}
\newcommand{\alr}[1]{\mute{\textcolor{ACMLightBlue}{(Albert: {#1})}}}
\newcommand{\is}[1]{\mute{\textcolor{ACMBlue}{(Ilya: {#1})}}}
\newcommand{\bl}[1]{\mute{\textcolor{ACMRed}{(Ben: {#1})}}}

\newcommand{\angled}[1]{\langle{#1}\rangle}
\newcommand{\set}[1]{\left\{{#1}\right\}}

\newcommand{\tname}[1]{\textsf{#1}\xspace}
\newcommand{\pname}[1]{\textsf{#1}\xspace}
\newcommand{\plname}[1]{\textsf{#1}\xspace}
\newcommand{\Coq}{\tname{Coq}}
\newcommand{\EVM}{EVM\xspace}
\newcommand{\evm}{EVM\xspace}
\newcommand{\keccak}{\ensuremath{\text{\code{KECCAK}}}\xspace}

\newcommand{\toolname}{\tname{\textsf{EVM2C}}} 

%Ben: Traductor: I think this is a super generic name--we need
%something more memorable

%\newcommand{\toolname}{\tname{Traductor}}

% Ilya: Traductor is nice, as it's a Spanish pun: "Oyente" -- "one
% who hears", "traductor" -- "one who interprets".

\newcommand{\solidity}{\plname{Solidity}}
\newcommand{\vyper}{\plname{Vyper}}
\newcommand{\oyente}{\tname{Oyente}}
\newcommand{\oyentestar}{\tname{Oyente*}}
\newcommand{\ethir}{\tname{EthIR}}
\newcommand{\ethirstar}{\tname{EthIR*}}
\newcommand{\SACO}{\tname{Saco}}
\newcommand{\PUBS}{\tname{Pubs}}
\newcommand{\COFLOCO}{\tname{Cofloco}}
\newcommand{\cpa}{\plname{CPAchecker}}
\newcommand{\verymax}{\plname{VeryMax}}
\newcommand{\seahorn}{\plname{SeaHorn}}
% Logic
\newcommand{\aand}{\wedge}
\newcommand{\oor}{\vee}

% Expressions
\newcommand{\unift}{\textit{unif}}
\newcommand{\unifi}{\textit{unif}}
%\newcommand{\lst}[1]{\mbox{\lstinline!#1!}}
\newcommand{\blockid}[1]{\ensuremath{blockId(#1)}}
\newcommand{\wset}[1]{\ensuremath{W(#1)}}

\newcommand{\proc}[1]{\hat{#1}}

\newcommand{\hbe}[1]{\ensuremath{\rightarrow_{#1}}\xspace}
\newcommand{\nhbe}[1]{\ensuremath{\nrightarrow_{#1}}\xspace}
\newcommand{\unif}{U_{\Rightarrow}}
\newcommand{\indep}[2]{I_{\bar{#1},\bar{#2}}}
\newcommand{\indepc}[2]{I_{{#1},{#2}}}
\newcommand{\back}{{\it back}}
\newcommand{\Sleep}{{\it Sleep}}
\newcommand{\sleep}{{\it sleep}}
\newcommand{\pre}{{\it pre}}
\newcommand{\notdep}{{\it notdep}}
\newcommand{\done}{{\it done}}

\newcommand{\algorithmicinput}{\textbf{Input:~}}
\newcommand{\algorithmicoutput}{\textbf{Output:~}}
\newcommand{\algorithmicglobal}{\textbf{Global:~}}

\newcommand{\key}[1]{\mbox{\ttfamily\bfseries #1}}
\newcommand{\last}{{\it last}}

\newcommand{\getBufferId}{{\it getActorId}}
\newcommand{\getTaskId}{{\it getTaskId}}


\newcommand{\getBuffer}{{\it getActor}}
\newcommand{\getTask}{{\it getTask}}



\newcommand{\nextS}{{\it next}}

\newcommand{\globals}{{\it G}}

%\newcommand{\Procedure}{Procedure}
\newcommand{\Explore}{{\it ModelCheck}}

% General commands
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\maxcard}{C^{max}}
\newcommand{\mincard}{C^{min}}
\newcommand{\initcontexts}[1]{\mathcal{I}^{#1}}
\newcommand{\inittasks}{\mathcal{T}_{ini}}
\newcommand{\classcard}[1]{|M_{C_{#1}}|}
%
% Commands for this paper
%\newcommand{\translate}{\tau}
\newcommand{\buffer}{\mathit{a}}
\newcommand{\queue}[0]{\C{Q}}
\newcommand{\microstepstar}[1]{\stackrel{#1}{\leadsto^*}}
\newcommand{\macrostep}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\newheap}{\ensuremath{newheap}}
%\newcommand{\C}[1]{{\cal #1}}
\newcommand{\rrderiv}{\leadsto}
\newcommand{\sepo}{\cdot}
\newcommand{\many}[1]{\overline{#1}}
\newcommand{\fut}{\mathit{fut}} 
\newcommand{\objset}{\ensuremath{\mathtt{Loc}}}
\newcommand{\futset}{\ensuremath{\mathtt{Fut}}}
\newcommand{\namemethod}{m}
\newcommand{\mapping}{l}
\newcommand{\heap}{h}
\newcommand{\dom}[0]{\ensuremath{\mathit{dom}}}
\newcommand{\tkset}{\ensuremath{\mathtt{T}}}
\newcommand{\future}{f}
\newcommand{\objid}[0]{\ensuremath{\mathit{o}}\xspace}
\newcommand{\Tkid}[0]{\ensuremath{\mathit{Tk}}\xspace}
\newcommand{\itable}[0]{\ensuremath{\mathit{IT}}\xspace}
\newcommand{\Objid}[0]{\ensuremath{\mathit{L}}\xspace}
\newcommand{\Futid}[0]{\ensuremath{\mathit{F}}\xspace}
\newcommand{\tkid}[0]{\ensuremath{\mathit{tk}}\xspace}
\newcommand{\timeid}[0]{\ensuremath{\mathit{t}}\xspace}
\newcommand{\lst}[1]{\lstinline!#1!}
\newcommand{\sst}[2]{\ensuremath{s(#1,#2)}\xspace}
\newcommand{\st}[4]{\ensuremath{s(#1,#2,#3,#4)}\xspace}
\newcommand{\rhotable}{\mbox{\emph{status}}}
\newcommand{\selectObject}{\ensuremath{\mathit{selectAct}}\xspace}
\newcommand{\selectTask}{\ensuremath{\mathit{selectTask}}\xspace}
\newcommand{\Await}[0]{\ensuremath{\mbox{\bf \lstinline!await!}}\xspace}
\newcommand{\get}[1]{\ensuremath{#1.\mbox{\bf \lstinline!get!}}\xspace}
\newcommand{\Get}[1]{\ensuremath{\mbox{\bf \lstinline!get!}}\xspace}
\newcommand{\newb}{\ensuremath{\mbox{\lstinline!new!}}\xspace}
\newcommand{\ifte}{\mbox{\lstinline!if!}\xspace}
\newcommand{\iftethen}{{\ensuremath{\mbox{\lstinline!then!}}\xspace}}
\newcommand{\ifteelse}{{\ensuremath{\mbox{\lstinline!else!}}\xspace}}
\newcommand{\while}{\mbox{\lstinline!while!}\xspace}
\newcommand{\whilebody}{\mbox{\lstinline!do!}\xspace}
\newcommand{\return}{\mbox{\lstinline!return!}\xspace}
\newcommand{\await}[1]{\mbox{\bf \lstinline!await!}~#1?\xspace}
\newcommand{\returnval}[1]{\mbox{\lstinline!return #1!}\xspace}
\newcommand{\body}[1]{\ensuremath{\mathit{body}(#1)}}
\newcommand{\nil}{\mbox{\lstinline!null!}\xspace}
\newcommand{\ex}{E}
\newcommand{\extend}[1]{S}
\newcommand{\exec}{{\it exec}}
\newcommand{\block}[1]{\ensuremath{#1.\mbox{\lstinline!block!}}}
\newcommand{\anndep}[1]{\ensuremath{\xrightarrow{#1}}}
\newcommand{\tktkdep}[0]{\ensuremath{\rightarrow}}
\newcommand{\abstkid}[0]{\ensuremath{\mathit{tk}}\xspace}
\newcommand{\ppset}{\ensuremath{\mathcal{P}}}
\newcommand{\pp}[1]{\ensuremath{\mathit{pp}(#1)}}
\newcommand{\taskpp}[2]{\ensuremath{{#1}{:}{#2}}}
\newcommand{\edge}[3]{\ensuremath{#1 \stackrel{_{#3}}{\longrightarrow} #2}}
\newcommand{\absobjid}[0]{\ensuremath{\mathit{ob}}\xspace}
\newcommand{\gdexec}[1]{{\it exec_{#1}}}
\newcommand{\deadlock}[1]{{\textsf{deadlock}(#1)}}

% CLP OPERATIONS
\newcommand{\newobject}{\texttt{new\_object}}
\newcommand{\getfield}{\texttt{get\_field}}
\newcommand{\setfield}{\texttt{set\_field}}
\newcommand{\mstep}{\texttt{mstep}}
\newcommand{\async}{\texttt{async}}
\newcommand{\getclp}{\texttt{get}}
\newcommand{\returnclp}{\texttt{return}}

\newcommand{\deps}[0]{\ensuremath{G}}
\newcommand{\absdeps}[0]{\ensuremath{\mathcal{G}}}
\newcommand{\ptresult}[0]{\ensuremath{\mathcal{A}}}

% Controlling the spaces
% \renewcommand{\topfraction}{0.998}
% \renewcommand{\textfraction}{0.01}
% \renewcommand{\floatpagefraction}{0.998}
\newcommand{\secbeg}{\vspace*{-0.15cm}}%-.15
\newcommand{\secend}{\vspace*{-0cm}}%-.15
\newcommand{\subsecbeg}{\vspace*{-0.1cm}}
\newcommand{\subsecend}{\vspace*{0cm}}

\newcommand{\taskId}{{\sf tk}}
\newcommand{\task}{\textsc{tk}}
\newcommand{\tv}{{\it l}}
%\newcommand{\state}[0]{S}
\newcommand{\futvar}[1]{{\tt #1_{\tt f}}}
\newcommand{\bufferId}{{\sf ac}}
\newcommand{\Fields}{{\it fields}}
\newcommand{\Refe}{{\sf Ref}}

\newcommand{\lot}[1]{\xoverline{l_{#1}}}
\newcommand{\sot}[1]{\xoverline{s_{#1}}}
\newcommand{\spot}[1]{\xoverline{s'_{#1}}}
\newcommand{\got}[1]{\xoverline{g_{#1}}}
\newcommand{\lvot}[0]{\xoverline{lv}}
\newcommand{\svot}[0]{\xoverline{sv}}
\newcommand{\blot}[0]{\xoverline{bc}}
\newcommand{\lpvot}[0]{\xoverline{lv'}}
\newcommand{\svpot}[0]{\xoverline{sv'}}
\newcommand{\blpot}[0]{\xoverline{bc'}}
\newcommand{\inot}[1]{\xoverline{i_{#1}}}
\newcommand{\svar}[1]{s_{#1}}
\newcommand{\spvar}[1]{s'_{#1}}
\newcommand{\invar}[1]{i_{#1}}
\newcommand{\gvar}[1]{g_{#1}}
\newcommand{\lvar}[1]{l_{#1}}
\newcommand{\lpvar}[1]{l'_{#1}}
\newcommand{\source}[1]{\textsf{#1}}
\newcommand{\sourcequoted}[1]{\lq\source{#1}\rq}


\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.7\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.7\mylenA\usebox\myboxB}%
    \fi}
\makeatother

\lstset{
  columns=flexible,
  frame=Ltb,
  framerule=0pt,
  aboveskip=0mm,
  framextopmargin=0pt,
  framexbottommargin=0pt,
  framexleftmargin=0cm,
  framesep=0pt,
  rulesep=0pt,
  % 
%   stringstyle=\ttfamily,
%   showstringspaces = false,
%   basicstyle=\small\bfseries,
%   commentstyle=\color{black},
%   keywordstyle=\small\bfseries,
  % 
  numbers=none,
  mathescape=true,
  numbersep=0pt,
  %numberstyle=\tiny,
  numberfirstline=true,
  numberblanklines=true,
  firstnumber=auto,
  breaklines=true,
  language=Java,
  basicstyle=\sffamily\scriptsize,
  keywordstyle=\sffamily\scriptsize\bfseries, 
  commentstyle=\sffamily\scriptsize\textit,
  numbers=left, 
  numberstyle=\sffamily\tiny,
  numbersep=4pt,
  morekeywords={function, contract, uint, mapping, struct,
  uint16, returns,
  if,then,else,while,do,await,block,get,cog,skip,release,begin,Int,Unit,Str,True,False,type,data,map,list,Map,List,Bool,Fut} }

\lstdefinestyle{numbers}
{numbers=left, numberstyle=\tiny}

\def\anno#1{{\ooalign{\hfil\raise.07ex\hbox{\small{\rm
          \textcolor{red}{{\tiny #1}}}}\hfil%
        \crcr{\scriptsize \textcolor{blue}{\mathhexbox20D}}}}}

\newcommand{\invalidLine}{\anno{!}}
\newcommand{\addedLine}{\anno{+}}

\newcommand{\change}[1]{\textcolor{blue}{#1}}
\newcommand{\changeJesus}[1]{\textcolor{red}{#1}}
\newcommand{\safevm}[1]{SAFEVM}

\newcommand{\pending}[1]{\textbf{\underline{#1}}\xspace}


%%%%%%%%%%% PLOTS %%%%%%%%%%%%%%%%%%%%%%

\definecolor{TRUE}{HTML}{00FF00}
\definecolor{UNKNOWN}{HTML}{FF0000}
\definecolor{TIMEOUT}{HTML}{add8e6}
\definecolor{ERROR}{HTML}{FFFFFF}

\pgfplotsset{
  percentage plot/.style={
    point meta=explicit,
    every node near coord/.append style={
      font=\tiny,
      color=black,
    },
    nodes near coords={
      \pgfmathtruncatemacro\iszero{\originalvalue==0}% <-- needed to remove space
      \ifnum\iszero=0
      \pgfmathprintnumber[fixed,fixed zerofill,precision=0]{\pgfplotspointmeta}
      \fi
    },
    yticklabel=\pgfmathprintnumber{\tick}\,$\%$,
    ymin=0,
    ymax=100.01, % added .01 
    visualization depends on={y \as \originalvalue},
    enlarge x limits={abs=6mm}
  },
  percentage series/.style={
    table/x expr=\coordindex, %added
    table/y expr=(\thisrow{#1}/\thisrow{sum}*100),
    table/meta=#1
    }
}


\newcommand{\statstable}[3]{
\begin{tikzpicture}[thick,scale=#3, every node/.style={scale=#3}]
\begin{axis}[
    ybar stacked,
    height=5cm,
    width=8cm,
    percentage plot,
    bar width=0.4cm, % increased from 0.3cm
    xticklabels from table={#2}{#1}, % read ticklabels from first column
    xtick=data,
    x tick label style={
      rotate=55,
      anchor=east, 
      xshift=-0.1mm, 
      yshift=-1.4mm
      %font=\small
    },
    y tick label style={
      font=\footnotesize
    }, 
    legend style={
      at={(0.5,-0.44)},
      anchor=south,
      legend columns=-1
      },
]
    \addplot [fill=TRUE]   table[percentage series=1] {#2};
    \addplot [fill=UNKNOWN]  table[percentage series=2] {#2};
    \addplot [fill=TIMEOUT]                 table[percentage series=3] {#2};
    \addplot [fill=ERROR]       table[percentage series=4] {#2};

    % plot just to add total
    \addplot [forget plot,nodes near coords align=above] table[x expr=\coordindex,y expr=0.0001,meta=sum]{#2};

    %\legend{\scriptsize{\strut TRUE}, \scriptsize{\strut UNKNOWN}, \scriptsize{\strut TIMEOUT}, \scriptsize{\strut ERROR}}
\end{axis}
\end{tikzpicture}
}

%% Termination plots

% \pgfplotstableread[col sep=comma,header=true]{plots/combinations-termin.csv}\combinationtermindata
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\combinationtermindata}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-uautomizer.csv}\tooluautomizer
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\tooluautomizer}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-cpa-termin.csv}\toolcpatermin
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\toolcpatermin}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-2ls.csv}\tooltwols
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\tooltwols}

% %% Reachability plots

% \pgfplotstableread[col sep=comma,header=true]{plots/combinations-reach.csv}\combinationreachdata
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\combinationreachdata}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-veriabs.csv}\toolveriabs
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\toolveriabs}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-cpa-reach.csv}\toolcpareach
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\toolcpareach}

% \pgfplotstableread[col sep=comma,header=true]{plots/tool-pesco.csv}\toolpesco
% \pgfplotstablecreatecol[
%  create col/expr={
%     \thisrow{1} + \thisrow{2} + \thisrow{3} +\thisrow{4}
%  }
% ]{sum}{\toolpesco}

\newcommand{\baseref}[0]{\ensuremath{\textit{baseref}}\xspace}
\newcommand{\offset}[0]{\ensuremath{\textit{offset}}}
\newcommand{\baserefs}[0]{\ensuremath{\textit{baserefs}}}
\newcommand{\getbaseref}[0]{\ensuremath{\textit{get\_baseref}}}
\newcommand{\getmemref}[0]{\ensuremath{\textit{get\_mem\_ref}}}
\newcommand{\isbaseref}[0]{\ensuremath{\textit{is\_baseref}}}
\newcommand{\isstatic}[0]{\ensuremath{\textit{is\_static}}}

\newcommand{\allbaserefs}[0]{\ensuremath\mathcal{M}}
\newcommand{\allstack}[0]{\ensuremath\mathcal{S}}
\newcommand{\absstate}[0]{\pi}
\newcommand{\transfer}[0]{\tau}
\newcommand{\absstatetop}[0]{\pi_{\top}}
\newcommand{\absstatebot}[0]{\pi_{\bot}}
\newcommand{\lub}{\sqcup}


\newcommand{\mem}[1]{$mem^{[#1]}$}
\newcommand{\slot}[1]{\textit{slot$_{#1}$}}
\newcommand{\opened}{\mathcal{O}}
\newcommand{\closed}{\mathcal{C}}
\newcommand{\closing}{\mathcal{K}}
\newcommand{\getslot}{\textit{get\_slots}}
\newcommand{\allslots}{\mathcal{A}}
\newcommand{\stackelems}{\mathcal{S}}
\newcommand{\stackset}{\mathcal{T}}
\newcommand{\programpoints}{\mathcal{P}}
\newcommand{\memelems}{\mathcal{M}}
\newcommand{\writeset}{\mathcal{W}}
\newcommand{\readset}{\mathcal{R}}
\newcommand{\writingleaks}{\mathcal{L}}
\newcommand{\reachable}{reachable\_from}
\newcommand{\existsread}{exists\_read}


==> running2-evm.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

\begin{figure}[t]
  \includegraphics[width=6.3cm]{running2-cfg.png}
\caption{Simplified CFG for \code{explicitOwnershipOf} in Example 2.}
\label{fig:running2-evm}
\end{figure}


==> running2.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%

%{\small \setlength\belowcaptionskip{-10pt}{
\begin{figure}[t]%\vspace{-1cm}

% \begin{center}
% \begin{tabular}{ll}

\begin{minipage}{6.5cm}
\begin{lstlisting}[name=running,firstnumber = 17, numbersep=6pt, language=Solidity]
contract Running2 {
  Running1 c;
  mapping(uint256 => uint256) private _packedOwnerships;

  function _ownershipAt(uint256 index) private view
$\slotcc{6}$      $\label{ex2:funchead3}$  returns (TokenOwnership memory) {
$\slotcc{7}$    $\label{ex2:externalcall}$return c.unpackedOwnership(_packedOwnerships[index]);
  }
\end{lstlisting}
\end{minipage}
%%%
\begin{minipage}{6cm}
  \begin{lstlisting}[name=running, numbersep=6pt, language=Solidity]
  $\label{ex2:funchead1}$  function explicitOwnershipOf(uint256 tokenId) public view
$\slotcc{3}$      $\label{ex2:funchead2}$      returns (TokenOwnership memory) {
$\slotcc{4}$  $\label{ex2:varres1}$    TokenOwnership memory ownership;
    if (...) {
$\label{ex2:return1}$$\slotcc{5}$  return ownership;
    }
$\slotcc{8}$    $\label{ex2:callres}$ownership = _ownershipAt(tokenId);
    //...
$\slotcc{5}$    $\label{ex2:return2}$return ownership;
  }
  //...
}
\end{lstlisting}
\end{minipage}
%   &
%     \begin{minipage}{4cm}
%       \includegraphics[scale=0.4]{cfg1.pdf}
%       \end{minipage}
%     \end{tabular}
% \end{center}
  %%

\begin{center}
\end{center}
  

\caption{\textsf{Solidity} code and memory representation for Example 2.}
\label{fig:running2}
\end{figure}


% Slot3: slot for returns variable (UNUSED)

% Slot4: local variable ownership (??)

% Slot5: slot to return the output struct: return of
% explicitOwnershipOf???.
% ***Common for both return sentences***

% Slot6: UNUSED (meaning???)   [[returns of _ownershipAt ???]]

% Slot7/Slot8: STATICCALL input/return values

% Slot9: return of _ownershipAt??? temporary copy of slot 8 to provide
% return in slot5 

       

